MegazordNet: combining statistical and machine learning standpoints for time series forecasting

Forecasting financial time series is considered to be a difficult task due to the chaotic feature of the series. Statistical approaches have shown solid results in some specific problems such as predicting market direction and single-price of stocks; however, with the recent advances in deep learning and big data techniques, new promising options have arises to tackle financial time series forecasting. Moreover, recent literature has shown that employing a combination of statistics and machine learning may improve accuracy in the forecasts in comparison to single solutions. Taking into consideration the mentioned aspects, in this work, we proposed the MegazordNet, a framework that explores statistical features within a financial series combined with a structured deep learning model for time series forecasting. We evaluated our approach predicting the closing price of stocks in the S&P 500 using different metrics, and we were able to beat single statistical and machine learning methods.

==> series_considered.tex <==

\begin{itemize*}[label={\tiny\raisebox{1ex}{\textbullet}}]
  \item MMM
  \item ABT
  \item ABBV
  \item ACN
  \item ATVI
  \item AYI
  \item ADBE
  \item AMD
  \item AAP
  \item AES
  \item AET
  \item AMG
  \item AFL
  \item A
  \item APD
  \item AKAM
  \item ALK
  \item ALB
  \item ARE
  \item ALXN
  \item ALGN
  \item ALLE
  \item AGN
  \item ADS
  \item LNT
  \item ALL
  \item GOOGL
  \item GOOG
  \item MO
  \item AMZN
  \item AEE
  \item AAL
  \item AEP
  \item AXP
  \item AIG
  \item AWK
  \item AMP
  \item ABC
  \item AME
  \item AMGN
  \item APH
  \item APC
  \item ADI
  \item ANDV
  \item ANSS
  \item ANTM
  \item AON
  \item AOS
  \item APA
  \item AIV
  \item AAPL
  \item AMAT
  \item ADM
  \item ARNC
  \item AJG
  \item AIZ
  \item T
  \item ADSK
  \item ADP
  \item AZO
  \item AVB
  \item AVY
  \item BLL
  \item BAC
  \item BK
  \item BCR
  \item BAX
  \item BBT
  \item BDX
  \item BRK.B
  \item BBY
  \item BIIB
  \item BLK
  \item HRB
  \item BA
  \item BWA
  \item BXP
  \item BSX
  \item BMY
  \item AVGO
  \item BF.B
  \item CHRW
  \item CA
  \item COG
  \item CPB
  \item COF
  \item CAH
  \item CBOE
  \item KMX
  \item CCL
  \item CAT
  \item CBG
  \item CBS
  \item CELG
  \item CNC
  \item CNP
  \item CTL
  \item CERN
  \item CF
  \item SCHW
  \item CHTR
  \item CHK
  \item CVX
  \item CMG
  \item CB
  \item CHD
  \item CI
  \item XEC
  \item CINF
  \item CTAS
  \item CSCO
  \item C
  \item CFG
  \item CTXS
  \item CLX
  \item CME
  \item CMS
  \item COH
  \item KO
  \item CTSH
  \item CL
  \item CMCSA
  \item CMA
  \item CAG
  \item CXO
  \item COP
  \item ED
  \item STZ
  \item COO
  \item GLW
  \item COST
  \item COTY
  \item CCI
  \item CSRA
  \item CSX
  \item CMI
  \item CVS
  \item DHI
  \item DHR
  \item DRI
  \item DVA
  \item DE
  \item DLPH
  \item DAL
  \item XRAY
  \item DVN
  \item DLR
  \item DFS.
\end{itemize*}
